Single-molecule Scale Nuclear Magnetic Resonance Spectroscopy using a Robust Near-Infrared Spin Sensor

Nuclear magnetic resonance (NMR) at the single-molecule level with atomic resolution holds transformative potential for structural biology and surface chemistry. Near-surface solid-state spin sensors with optical readout ability offer a promising pathway toward this goal. However, their extreme proximity to target molecules demands exceptional robustness against surface-induced perturbations. Furthermore, life science applications require these sensors to operate in biocompatible spectral ranges that minimize photodamage. In this work, we demonstrate that the PL6 quantum defect in 4H silicon carbide (4H-SiC) can serve as a robust near-infrared spin sensor. This sensor operates at tissue-transparent wavelengths and exhibits exceptional near-surface stability even at depth of 2 nm. Using shallow PL6 centers, we achieve nanoscale NMR detection of proton ($\mathrm{^{1}H}$) spins in immersion oil and fluorine ($\mathrm{^{19}F}$) spins in Fomblin, attaining a detection volume of $\mathrm{(3~nm)^3}$ and a sensitivity reaching the requirement for single-proton spin detection. This work establishes 4H-SiC quantum sensors as a compelling platform for nanoscale magnetic resonance, with promising applications in probing low-dimensional water phases, protein folding dynamics, and molecular interactions.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdfxe'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
